Solving Short-Term Relocalization Problems In Monocular Keyframe Visual SLAM Using Spatial And Semantic Data

In Monocular Keyframe Visual Simultaneous Localization and Mapping (MKVSLAM) frameworks, when incremental position tracking fails, global pose has to be recovered in a short-time window, also known as short-term relocalization. This capability is crucial for mobile robots to have reliable navigation, build accurate maps, and have precise behaviors around human collaborators. This paper focuses on the development of robust short-term relocalization capabilities for mobile robots using a monocular camera system. A novel multimodal keyframe descriptor is introduced, that contains semantic information of objects detected in the environment and the spatial information of the camera. Using this descriptor, a new Keyframe-based Place Recognition (KPR) method is proposed that is formulated as a multi-stage keyframe filtering algorithm, leading to a new relocalization pipeline for MKVSLAM systems. The proposed approach is evaluated over several indoor GPS denied datasets and demonstrates accurate pose recovery, in comparison to a bag-of-words approach.

==> sections/Notation.tex <==
\section{Notations and Conventions}
\label{sec:notation}
In this section, we define the notation conventions used throughout the paper. Data structures are represented by the calligraphic capital letter \( \mathcal{D}\) showing only those variables relevant to the problem. Scalars are represented using normal-face letters \( A, a \). Vectors and Matrices are represented using bold-face letters \( \mathbf{B} \), \( \mathbf{b} \). Lists are represented as either \( \{ A_m^i \} \) or \( \{ a_m \} \), where \( m \) represents the timestep and \( i \) shows the number of elements. Elements of a matrix are denoted by \( a_{ij} \) where \( i \) and \( j \) are the row and column indices respectively. The matrix norm is denoted as \(||.||_p\) where $p$ is the chosen norm. Scalar, matrix/vector, and list variables of a data structure are represented as $\mathcal{D}.A$, $\mathcal{D}.\mathbf{B}$, $\mathcal{D}.\{ A_m^i \}$ respectively. 



% Add more as we finish writing section IV


% ---------------- Section End -------------------------------------------------------

  
% Math command nodes
% \( \mathcal{F}_n \) -- Caligraphic F with n subscript
% \( \mathcal{F}_n = \{{\mathbf{S_n}, \mathbf{I_n}}\} \) command for a data structure
% \( \mathbf{I}_n \)
% \( \{ x_j \} \)
